Separation of Powers in Federated Learning

Federated Learning (FL) enables collaborative training among mutually distrusting parties. Model updates, rather than training data, are concentrated and fused in a central aggregation server. A key security challenge in FL is that an untrustworthy or compromised aggregation process might lead to unforeseeable information leakage. This challenge is especially acute due to recently demonstrated attacks that have reconstructed large fractions of training data from ostensibly "sanitized" model updates. In this paper, we introduce TRUDA, a new cross-silo FL system, employing a trustworthy and decentralized aggregation architecture to break down information concentration with regard to a single aggregator. Based on the unique computational properties of model-fusion algorithms, all exchanged model updates in TRUDA are disassembled at the parameter-granularity and re-stitched to random partitions designated for multiple TEE-protected aggregators. Thus, each aggregator only has a fragmentary and shuffled view of model updates and is oblivious to the model architecture. Our new security mechanisms can fundamentally mitigate training reconstruction attacks, while still preserving the final accuracy of trained models and keeping performance overheads low.

==> Makefile <==
NAME=main

TARGET=$(NAME)
BIBTEX := bibtex
TGIF   := tgif
XFIG   := xfig
GNUPLOT:= gnuplot

SOURCES=$(wildcard *.tex) $(wildcard *.bib)

FIGS= $(wildcard figures/*)

all: $(TARGET).pdf
$(TARGET).pdf: Makefile  $(SOURCES) $(FIGS)
	pdflatex  $(TARGET).tex
	-bibtex --min-crossrefs=100    $(TARGET)
	pdflatex  $(TARGET).tex
	pdflatex  $(TARGET).tex

color: $(TARGET).pdf
	pdflatex $(TARGET).tex
	pdftops $(TARGET).pdf

$(TARGET).ps: $(TARGET).pdf
	pdflatex "\newcommand{\wantBW}{} \input{$(TARGET).tex}"
	pdftops $(TARGET).pdf

%.pdf : %.fig #Makefile
	fig2dev -L pdf -b 1 $< $@

%.eps : %.dia #Makefile
	dia --nosplash -e $@ $<

%.eps : %.obj
	TMPDIR=/tmp $(TGIF) -print -eps $<

%.pdf : %.eps #Makefile
	epstopdf $<

check:
	grep -nr "ﬂ\|ﬁ" .
	grep -nr "“" .
	grep -nr "’" .

clean:
	rm -f *.aux *.log *.out *.bbl *.blg *~ $(TARGET).dvi $(TARGET).pdf
